Specifying a Realistic File System

We present the most interesting elements of the correctness specification of BilbyFs, a performant Linux flash file system. The BilbyFs specification supports asynchronous writes, a feature that has been overlooked by several file system verification projects, and has been used to verify the correctness of BilbyFs's fsync() C implementation. It makes use of nondeterminism to be concise and is shallowly-embedded in higher-order logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{R.J. van Glabbeek, J.F. Groote \& P. H\"ofner (Eds.):
Workshop on\\
Models for Formal Analysis of Real Systems (MARS 2015)\\
EPTCS 196, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.196.1}{10.4204/EPTCS.196.1}}
\pdfoutput=1

